Generalized Parametric Contrastive Learning

In this paper, we propose the Generalized Parametric Contrastive Learning (GPaCo/PaCo) which works well on both imbalanced and balanced data. Based on theoretical analysis, we observe that supervised contrastive loss tends to bias high-frequency classes and thus increases the difficulty of imbalanced learning. We introduce a set of parametric class-wise learnable centers to rebalance from an optimization perspective. Further, we analyze our GPaCo/PaCo loss under a balanced setting. Our analysis demonstrates that GPaCo/PaCo can adaptively enhance the intensity of pushing samples of the same class close as more samples are pulled together with their corresponding centers and benefit hard example learning. Experiments on long-tailed benchmarks manifest the new state-of-the-art for long-tailed recognition. On full ImageNet, models from CNNs to vision transformers trained with GPaCo loss show better generalization performance and stronger robustness compared with MAE models. Moreover, GPaCo can be applied to the semantic segmentation task and obvious improvements are observed on the 4 most popular benchmarks. Our code is available at https://github.com/dvlab-research/Parametric-Contrastive-Learning.

==> Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := TPAMI-PaCo

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex


clean:
	rm -rf *.log *.aux *.blg *.bbl *.gz *.dvi *.thm *.dat *.out *latexmk *fls *busy\)



==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> doc/bio.tex <==
\vspace{-0.1in}
\begin{IEEEbiography}
[{\includegraphics[height=1.26in,clip,keepaspectratio]
    {bio_fig/jiequan_cui.jpg}}]
{Jiequan Cui}
received the B.Eng.~degree from the Computer Science Department of ShanDong University (SDU) in 2018 and the Ph.D.~degree from The Chinese University of Hong Kong (CUHK) in 2022.
He is currently a research fellow in the School of Computer Science and Engineering (SCSE), Nanyang Technological University (NTU).
He serves as a reviewer for TPAMI, IJCV, TIP, CVPR, ICCV, ECCV, ICLR, NeurIPS, and ICML. His research interests include model generalization and robustness, imbalanced learning, adversarial robustness, neural architecture search, and image segmentation.
\end{IEEEbiography}

\vspace{-0.1in}
\begin{IEEEbiography}
[{\includegraphics[height=1.25in,clip,keepaspectratio]
    {bio_fig/Zhisheng_Zhong.jpg}}]
{Zhisheng Zhong}
received the B.Eng. Degree in Communication Engineering from Beijing University of Posts and Telecommunications (BUPT) in 2016. He received the Master Degree in Computer Science from Peking University (PKU) in 2019. Now he is a Ph.D. student at the Department of Computer Science Engineering~(CSE), the Chinese University of Hong Kong (CUHK). He serves as a reviewer for NeurIPS, CVPR, ICCV, ICLR and etc. His research interests lie in deep learning and computer vision.
\end{IEEEbiography}

\vspace{-0.1in}
\begin{IEEEbiography}
[{\includegraphics[height=1.25in,clip,keepaspectratio]
    {bio_fig/zhuotao_tian.jpg}}]
{Zhuotao Tian} is currently a researcher at SmartMore. He
received the B.Eng. degree (Honors) from Harbin Institute of Technology (HIT) in 2018, and obtained the Ph.D. degree in 2022, from the Chinese University of Hong Kong (CUHK), under the supervision of Prof. Jiaya Jia and Prof. Bei Yu. He serves as a reviewer for top nenues including TPAMI, CVPR, ICCV, ECCV, ICML, ICLR, NeurIPS, AAAI, IJCV and TIP. His research interests include broad topics related to general 2D-3D semantic segmentation, few-shot learning, and semi-supervised learning.
\end{IEEEbiography}

\vspace{-0.1in}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]
    {bio_fig/shu_liu}}]
{Shu Liu}
now serves as Co-Founder and Technical Head in SmartMore. He received the BS degree from Huazhong University of Science and Technology and the PhD degree from the Chinese University of Hong Kong. He was the winner of 2017 COCO Instance Segmentation Competition and received the Outstanding Reviewer of ICCV in 2019. He continuously served as a reviewer for TPAMI, CVPR, ICCV, NeurIPS, ICLR and etc. His research interests lie in deep learning and computer vision.
\end{IEEEbiography}	

\vspace{-0.1in}
\begin{IEEEbiography}
[{\includegraphics[height=1.25in,clip,keepaspectratio]{bio_fig/byu.pdf}}]{Bei Yu}
(Member, IEEE)
    received the Ph.D.~degree from The University of Texas at Austin in 2014.
    He is currently an Associate Professor in the Department of Computer Science and Engineering, The Chinese University of Hong Kong.
    He has served as TPC Chair of ACM/IEEE Workshop on Machine Learning for CAD, and in many journal editorial boards and conference committees.
    He is Editor of IEEE TCCPS Newsletter.
    He received nine Best Paper Awards from DATE 2022, ICCAD 2021 \& 2013, ASPDAC 2021 \& 2012, ICTAI 2019, Integration, the VLSI Journal in 2018, ISPD 2017,
    SPIE Advanced Lithography Conference 2016, and six ICCAD/ISPD contest awards.
    \end{IEEEbiography}

    \begin{IEEEbiography}
    [{\includegraphics[height=1.25in,clip,keepaspectratio]{bio_fig/jiaya_jia}}]
{Jiaya Jia}
received the Ph.D.~degree in Computer Science from Hong Kong University of Science and Technology in 2004 and is currently a full professor in Department of Computer Science and Engineering at the Chinese University of Hong Kong (CUHK). He assumes the position of Associate Editor-in-Chief of IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI) and is in the editorial board of International Journal of Computer Vision (IJCV). He continuously served as area chairs for ICCV, CVPR, AAAI, ECCV, and several other conferences for the organization. He was on program committees of major conferences in graphics and computational imaging, including ICCP, SIGGRAPH, and SIGGRAPH Asia. He is a Fellow of the IEEE. 
V\end{IEEEbiography}



==> doc/cover.tex <==
{
%\twocolumn[
%\begin{@twocolumnfalse}
%\large

\noindent Dear Editors,

\noindent
Our submission ``Generalized Parametric Contrastive Learning'' to TPAMI is an extension of our conference paper published at ICCV 2021. The changes are intensive, as summarized in the following.

\noindent
\vspace{0.2cm} \ \\ 
\textbf{Change 1:} We examine the necessary of each component (augmentation strategy, formulation of PaCo, the momentum encoder and queue size) in PaCo and simplify Parametric Contrastive Learning (PaCo) to Generalized Contrastive Learning (GPaCo) by removing the momentum encoder. GPaCo outperforms PaCo by a large margin. We verify the generality of GPaCo on various tasks, including long-tailed recognition, recognition on full ImageNet and CIFAR-100 datasets, robustness on out-of-distribution data, and semantic segmentation. 


\vspace{0.2cm} \ \\
\noindent
\textbf{Change 2}: We validate that GPaCo can improve model generalization ability and robustness on out-of-distribution data varying from CNNs (ResNet) to vision transformers (ViT models) when compared with MAE models.  

\noindent (I) For robustness on out-of-distribution data, 
with ViT-B, GPaCo models obtain respectively \textbf{2.6\%}, \textbf{1.8\%}, \textbf{3.3\%} improvement on ImageNet-C, ImageNet-R, and ImageNet-S.
With ViT-L, GPaCo models obtain \textbf{2.4\%} and \textbf{2.8\%} improvement on ImageNet-C and ImageNet-S, respectively.

\noindent (II) On full ImageNet, GPaCo models outperform baselines, {\textit i.e.}, MAE models, by \textbf{0.4} and \textbf{0.3} with ViT-B and ViT-L respectively.


\vspace{0.2cm} \ \\
\noindent
\textbf{Change 3}: We transfer GPaCo to the downstream task, {\textit i.e.}, semantic segmentation. Taking GPaCo as an auxiliary loss, obvious improvement is observed on popular semantic segmentation benchmark of ADE20K, COCO-Stuff, PASCAL Context and Cityscapes.

\noindent (I) On ADE20K, we experiment with swin transformer and upernet. improvement is yielded from Swin-T to Swin-L models when equipped with GPaCo, outperforming baselines by \textbf{1.0}, \textbf{1.5}, and \textbf{0.8} mIoU respectively.

\noindent (II) On PASCAL Context, GPaCo models significantly surpass baselines by \textbf{1.6} and \textbf{1.7} mIoU with ResNet-50 and ResNet-101 respectively.

\noindent (III) On COCO-Stuff, GPaCo models significantly surpass baselines by \textbf{1.1} and \textbf{1.1} mIoU with ResNet-50 and ResNet-101 respectively.

\noindent (IV) On Cityscapes, GPaCo models outperforms baselines by \textbf{0.9} and \textbf{0.9} mIoU with ResNet-18 and ResNet-50 individually.


\noindent
\vspace{0.2cm} \ \\
\textbf{Change 4}: We add several ablation experiments to explore the mechanism of GPaCo.

\noindent (I) Comprehensive comparisons between GPaCo/PaCo and multi-task learning on long-tailed data, {\textit i.e.}, ImageNet-LT.

\noindent (II) Comprehensive comparisons between GPaCo/PaCo and multi-task learning on balanced data, {\textit i.e.}, full CIFAR-100 and full ImageNet.

\noindent (III) Ablation on model ensemble with GPaCo models for imbalanec data.

\noindent (IV) Ablation on effects of queue length of GPaCo.

\noindent (V) Ablation on the necessary of two views training of GPaCo.

%\end{@twocolumnfalse}
%]
}

